Adaptive MapReduce Similarity Joins

Similarity joins are a fundamental database operation. Given data sets S and R, the goal of a similarity join is to find all points x in S and y in R with distance at most r. Recent research has investigated how locality-sensitive hashing (LSH) can be used for similarity join, and in particular two recent lines of work have made exciting progress on LSH-based join performance. Hu, Tao, and Yi (PODS 17) investigated joins in a massively parallel setting, showing strong results that adapt to the size of the output. Meanwhile, Ahle, Aum\"uller, and Pagh (SODA 17) showed a sequential algorithm that adapts to the structure of the data, matching classic bounds in the worst case but improving them significantly on more structured data. We show that this adaptive strategy can be adapted to the parallel setting, combining the advantages of these approaches. In particular, we show that a simple modification to Hu et al.'s algorithm achieves bounds that depend on the density of points in the dataset as well as the total outsize of the output. Our algorithm uses no extra parameters over other LSH approaches (in particular, its execution does not depend on the structure of the dataset), and is likely to be efficient in practice.

==> buckets.tex <==
\section{Processing Buckets Efficiently}
\seclabel{buckets}

In this section, we show that buckets can be efficiently processed in the Mapreduce, I/O, and BSP models.

This section is divided into several subsections, one for each model.  In each subsection, we briefly summarize the model and the lower bound, then describe a simple way to process buckets to reach this lower bound.

As mentioned earlier, in each case, our algorithm can likely be substituted or combined with previous work on the model. This can be particularly efficient if the previous work has tight analysis for a particular distance metric. For example, \cite{} may give improved performance for MapReduce bucket processing under the hamming metric.

\subsection{MapReduce}

\subsection{External Memory}
As mentioned in \cite{}, we can essentially hope to do at most $MB$ pairwise comparisons per I/O.  Thus, we want to spend at most $\frac{1}{MB} \sum_i \text{comparisons}(B_i)$ I/Os to compute the pairwise joins.

Note that hashing incurs a significant cost in this model.  In particular, we require $\sum_i \lceil |B_i|/B\rceil$ I/Os just to hash the elements.  We show that a small modification of the original algorithm can take this cost into account.

In particular, if the cost of hashing is high\footnote{In particular, if each element is compared to less than $M$ elements on average in our buckets}, our algorithm balances the cost of TODO.
%, meeting the bounds of \cite{TODO} in the worst case.  
Otherwise, we obtain the same performance we did in the other models.

TODO: compare our results for ESA.  If the buckets are relatively dense we actually win even in the worst case (from an easy analysis).  Otherwise, we get similar bounds, but we're more data-dependent.  Give examples of each.

\subsection{BSP}


==> em.tex <==
\section{I/O efficient similarity join}


==> lsh.tex <==
%\section{Creating Buckets with Data-Dependent LSH}
\section{Data-Dependent LSH To Filter Out Far Pairs}
\seclabel{lsh}

We present our algorithm in this section.  We begin with a high-level overview, then give a more detailed description of how to run the algorithm.  Finally, we analyze the algorithm and prove our performance bounds.

Our algorithm is parameterized by a factor $\epsilon = \Omega((\log n)/M)$.  This value gives a minor tradeoff between the expected performance of the algorithm and its concentration bounds.

Our algorithm:  
\begin{itemize}
    \item Hash all points with $\log n$ LSH's to obtain a hash function $\hat{h}$; distribute them in order among machines
    \item Combine points to get buckets of size $O(M)$.
    \item Count the size of all buckets at higher levels using the parallel summing technique.  Let $B_k(x)$ be the size of the bucket at level $k$ containing $x$.
    \item Calculate $\hat{W}(x) = \min_k B_k(x)/p_1^k + M/p_1^k$  \sam{I don't think we need the plus term}
    \item Let $K(x) = \{k ~|~ B_k(x)/p_1^k + M/p_1^k \leq (1 + \epsilon) \hat{W}(x)\}$.  
    \item Hash $x$ at level $\alpha(x) = 1 + \min K(x)$. 
    \item For each $x$, create $\alpha(x)$ copies of $x$ (one for each level).  
    \item For each bucket at level $k$, compare all elements in $R$ with level $k$ with all elements in $S$ and vice versa.  
\end{itemize}

\subsection{Round 1: Sampling}

In this section, we prove \sam{sampling theorem}---in other words, we show how to find $\alpha(x)$ for all $x\in R\cup S$ with $O(1)$ rounds and $O(N/p)$ load.

First concatenate $\log n$ hash functions to get $\hat{h}$.  For each $x\in R\cup S$, create a pair $(x,\hat{h}(x))$; sort these pairs in $O(1)$ rounds using \sam{sorting ref}.  

Now, we obtain the smallest possible buckets of size $> M$.

\subsection{Round 2: Comparing}


\subsection{Analysis}

We bound the expected performance of our sampled level for any point $x\in R$.  A mirrored argument gives the same bound for each $y\in S$.

\begin{lemma}
    In expectation, the cost of hashing a point at level $\alpha(x)$ is within a constant factor of optimal.  In other words, for all $x\in R$, 
    \[
        \E_{\hat{h}} \left[ \sum_{y\in S} \left(\frac{\Pr(h(x) = h(y))}{p_1}\right)^{\alpha(x)} + \frac{M}{p_1^{\alpha(x)}}\right] = O(W(x,S)).
    \]
\end{lemma}
\begin{proof}
    Let $\ell(x)$ be the {optimal level} to hash $x$. We refer to $\ell(x)$, $K$, and $\alpha(x)$ as $\ell$, $K$, and $\alpha$ for simplicity.  We ignore the $M/p_1^k$ term in our analysis; this affects our bounds by at most a constant factor.  We repeatedly assume that $\epsilon$ is small enough that $1/(1 + \epsilon) \approx 1 - \epsilon$.

    %For simplicity, we do not try to optimize constants in this proof.  Since we assume $M > N^{\epsilon}$, all constants can be replaced by $1 + \epsilon'$ for subconstant $\epsilon'$ without affecting correctness.

    First, we show that $\ell \in K$ with high probability.  Since $\E [B_{\ell}(x)/{p_1}^{\ell}] = W(x,S)$, we have $B_{\ell}(x)/p_1^{\ell} < (1 + \epsilon/2)W(x,S)$ with probability at least $1 - e^{-\epsilon^2 M/12}$ (since $\E[B_{\ell}]\geq M$) via Chernoff bounds.  
    Similarly, for any other level $k$, $\E[B_k/p_1] \geq W(x,S)$, so $B_k(x)/p_1^k \geq (1 - \epsilon/2) W(x,S)$ with probability at least $1 - e^{-\epsilon^2 M/8}$.  
    %Because $1 + \epsilon \approx (1 + \epsilon/2)/(1 - \epsilon/2)$ and 
    We assumed $\epsilon^2 M  = \Omega(\log n)$, so $\ell\in K$ with high probability.
    We also immediately obtain $\hat{W}(x) \leq (1 + \epsilon/2) W(x,S)$  with high probability.
    %Because $M = \Omega(\log n)$, we have $\ell\in K$ with high probability.  

    Because $\ell\in K$ and we choose the highest level in $K$, we must choose a level that is $\ell$ or higher.  We now bound the expected cost of choosing a level $k > \ell$.  We split into two cases, based on $\E[B_k/p_1^k]$.

    First, assume $\E[B_k/p_1^k] \geq (1+\epsilon)^2 W(x,S)$. 
    %\[ \sum_{y\in S} \left(\frac{\Pr(h(x) = h(y))}{p_1}\right)^k \geq 36W(x,S).  \]
    Then $B_k/p_1^k \leq (1+\epsilon) W(x,S)$ with probability at most $e^{-\epsilon^2 M/8}$.  Since we showed $\hat{W}(x) \leq (1 + \epsilon/2) W(x,S)$ with high probability, $k\notin K$ with high probability.

    Otherwise, assume $\E[B_k/p_1^k] \leq (1 + \epsilon)^2 W(x,S)$.  
    Then if we select $k$, we obtain expected cost at most $(1 + \epsilon)^2 W(x,S) = O(W(x,S))$.  
\end{proof}

\begin{proof}
    %By definition of the algorithm, the Equi-Join outputs each pair of elements in each bucket.  Thus, we immediately obtain 
    Consider an element $x\in R$ at (sampled) level $\alpha(x)$.   Then during the Equi-Join operation, $x$ will be compared to all $y\in S$ in every bucket containing $x$ at level $\alpha(x)$.   Thus, every pair output by the equi-join has one element $x$ at level $\alpha(x)$; we charge the pair to that element $x$.  
    
    
    Thus, we immediately obtain $\AOUT(R,S,r) \leq \E[\sum_{x\in S} W(x,S) + \sum_{y\in S} W(y,R)]$.

    We now bound the cost of the equi-join.  Consider a bucket $B$ with input size (i.e. total number of elements) $B_{\IN}$ and output size $B_{\OUT}$.  We want to show that $B_{\IN} = O(\sqrt{B_{\OUT}})$.  First, assume that 
\end{proof}

\begin{lemma}
    If $x\in R$ and $y\in S$ with $d(x,y)\leq r$, then \sam{$x$ and $y$ are compared in the equijoin step.} with constant probability.

    Using $\Theta(\log n)$ parallel repetitions of our algorithm, $x$ and $y$ are compared in at least one repetition with high probability.  This increases the load factor of \sam{performance theorem} by a factor $\Theta(\log n)$.
\end{lemma}

\begin{proof}
    Let $\alpha = \max\{\alpha(x),\alpha(y)\}$ be the level where $x$ and $y$ are compared.\footnote{We take the max because $x$ (resp. $y$) is only compared in buckets at level $\alpha(x)$ (resp. $\alpha(y)$) or higher.}  We compare $x$ and $y$ if they are in the same bucket at level $\alpha$.  Because our hash functions are independent, $x$ and $y$ collide at level $\alpha$ with probability $\Pr(h(x) = h(y))^\alpha \geq p_1^{\alpha}$.  We hash each item to $1/p_1^{\alpha}$ buckets, so $x$ and $y$ collide in at least one with probability $1 - (1 - p_1^{\alpha})^{1/p_1^{\alpha}} = \Omega(1)$.

    Over $\Theta(\log n)$ repetitions, $x$ and $y$ are \sam{compared in the equijoin step} with high probability using standard Chernoff bounds.  The increased load factor for the parallel repetitions follows via linearity of expectation.  
\end{proof}

%\sam{After here is deprecated}
%
%\begin{lemma}
%    For a given $x$, let $k'$ solve $\sum \Pr(h(x) = h(y))^{k'} = M$.  Then $k(x) = \lfloor k'\rfloor$ or $k(x) = \lceil k'\rceil$.
%\end{lemma}
%\begin{proof}
%    Convexity.
%\end{proof}
%
%\begin{lemma}
%    Let $\hat{W}(x)$ be the number of points compared to $x$ at level $\hat{x}(x)$.  Then $\E[\hat{W}(x)] = O(W(x))$.
%\end{lemma}
%\begin{proof}
%    We split into two cases based on the optimal number of comparisons.
%
%    In the first case, there exists a $k'$ such that $\sum \Pr(h(x) = h(y))^{k'} \in [M/2, 2M]$.   \sam{Let's assume that $k'$ is optimal for now.  I think we can show that $k(x) \leq k' + 1 \leq k(x) + 1$.}  First, using Chernoff bounds, the probability that level $k$ has more than $6M$ elements is at most $e^{-2M/3}$; similarly, the probability that level $k$ has less than $M/4$ elements is at most $e^{-M/8}$.  Since $M > \log n$, we select $k'$ or a higher level with high probability.
%
%    Consider a level $k'' < k$.  Let $\sum \Pr(h(x) = h(y))^{k'} = C \geq 12M$.  Then, again by Chernoff, level $k''$ has at most $6M$ elements with probability $e^{-C/8}.$
%
%    If we select a level $k'' < k$ with cost $C < 12M$, the total cost is $13M/b_1^{k''} \leq 12M/b_1^k = O(W(x))$.  The expected cost of all other levels is at most $\sum_{k'' < k} C/b_1^{k''} e^{-C/8} \leq 1/b_1^k = O(W(x))$. 
%
%    In the second case, there is no level in the range $[M/2, 2M]$.  Let $k'$ be the smallest-index level with less than $M$ elements in expectation.  Using Chernoff bounds, all $k'' < k'$ have at least $M$ elements with probability at most $e^{-M/8}$.  Similarly, all $k'' \geq k$ have at most $M$ elements with probability at most $e^{-M/3}$.  Thus, we return $k'$ with high probability.  By definition, $\Pr(h(x) = h(y))^{k'} \leq W(x)/p_1 = O(W(x))$.  
%\end{proof}

